Gen2Sim: Scaling up Robot Learning in Simulation with Generative Models

Generalist robot manipulators need to learn a wide variety of manipulation skills across diverse environments. Current robot training pipelines rely on humans to provide kinesthetic demonstrations or to program simulation environments and to code up reward functions for reinforcement learning. Such human involvement is an important bottleneck towards scaling up robot learning across diverse tasks and environments. We propose Generation to Simulation (Gen2Sim), a method for scaling up robot skill learning in simulation by automating generation of 3D assets, task descriptions, task decompositions and reward functions using large pre-trained generative models of language and vision. We generate 3D assets for simulation by lifting open-world 2D object-centric images to 3D using image diffusion models and querying LLMs to determine plausible physics parameters. Given URDF files of generated and human-developed assets, we chain-of-thought prompt LLMs to map these to relevant task descriptions, temporal decompositions, and corresponding python reward functions for reinforcement learning. We show Gen2Sim succeeds in learning policies for diverse long horizon tasks, where reinforcement learning with non temporally decomposed reward functions fails. Gen2Sim provides a viable path for scaling up reinforcement learning for robot manipulators in simulation, both by diversifying and expanding task and environment development, and by facilitating the discovery of reinforcement-learned behaviors through temporal task decomposition in RL. Our work contributes hundreds of simulated assets, tasks and demonstrations, taking a step towards fully autonomous robotic manipulation skill acquisition in simulation.

==> 3_method_xian.tex <==
\begin{figure*}[!htb]
    \centering
     \begin{subfigure}[b]{0.3\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{draft_figures/image_to_3d_method.png}
         \label{fig:method_img_to_3d}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{graph1}
         \label{fig:llm_prompting}
     \end{subfigure}
     \hfill
    \caption{\textbf{Left: Image to 3D Pipeline}  \textbf{Right: Environment to reward generation pipeline}}
    \label{fig:pipeline}
\end{figure*}

\section{\model{}}
%\todo{The method section should be written independent of the simulator environments}

% \todo{The overview for \model{} is shown in Figure \ref{fig:architecture}.} 
\model{} generates 3D assets from object images using image diffusion models and predicts physical parameters for them using LLMs (Section \ref{sec:assets}). It then prompts LLMs to generate language task descriptions and corresponding reward functions for each generated or human-developed asset,  suitable to their affordances (Section \ref{sec:prompting}). Finally, we train RL policies in the generated environments using the generated reward functions, allowing robots to acquire manipulation skills in diverse scenes and tasks. We additionally show the applicability of the simulation trained policy by constructing digital twin environment in simulation, and deploy the trained trajectory in the real world (Section \ref{sec:RL}). 

\input{assets}
%\todo{PUSHKAL-XIAN: can you write down the queries to GPR4?}

% \begin{comment}
% \begin{figure}[h!]
%     \centering
%     \includegraphics[height=13cm,keepaspectratio]{draft_figures/assets3dcreated}
%     \caption{\textbf{3D asset generation from vision and language generative models.} Given a real or generated seed image, our method lifts it in 3D using score distillation sampling  under a cross-view and pose-conditioned image diffusion model. We show two rendered views of the resulting 3D assets in actual relative 3D size predicted by the LLM. We further show twin simulation environments created by lifting each object in the scene, one by one.}
%     \label{fig:assets3dcreated}
% \end{figure}
% \end{comment}
% \vspace{-0.05in}


\subsection{Task Decomposition and Reward Generation with LLMs} \label{sec:prompting}
%\vspace{-0.05in}


Given the simulation assets and their URDFs, we prompt GPT-4 \cite{openai2023gpt4} to generate meaningful tasks, together with their language descriptions and reward functions. 

%We design chain-of-thought \cite{wei2023chainofthought} prompts with in-context examples to elicit reasoning while generating tasks and reward functions. Moreover, such a prompting style also provides structure to generations, useful for parsing relevant content in downstream programs for automation. The in-context example consists of the following components:  

\paragraph{Environment Description} A list of assets with their structural details including parts with their links, and joints with their types, and limits. We extract these details from the URDF in an automated fashion using scripts. For example, an asset "Dishwasher" with parts ["door", "handle" and "body"], and joint ["door-joint"] of type revolute with a range between [0, 1]. Such context allows LLM to reason about relevant parts and joints of assets in the simulation environment. Moreover, such part-level details of the asset enable LLM to reason about the affordances relevant to manipulation tasks.

\paragraph{Tasks and Corresponding Reward Functions} A list of meaningful tasks with their language descriptions and reward functions. Each task contains a language description, and a corresponding reward function describing the reward logic and success condition to achieve the task. Such examples provide the LLM context to perform reasoning to generate meaningful task language descriptions and appropriate reward functions. For example, meaningful manipulation tasks in an environment with Dishwasher are opening and closing the Dishwasher door. For the door opening/closing task, the part-aware reward functions contain three terms: (i.) Distance Reward: distance between the end-effector and the target part handle (ii.) Part-State Reward: error between the current and the target pose of the articulated door. (iii.) Grasp Reward: grasping the handle of the door. The complete reward function is as follows:
\begin{equation}
\label{eq:reward}
\lambda_d R_{\text {dist}}+\lambda_p R_{\text {pose}}+\lambda_t R_{\text {grasp}}
\end{equation}

Real-world manipulation tasks can also have long horizons and can be decomposed into different levels of granularity for execution. Prior works have shown that LLMs can perform task decompositions \cite{saycan, etc?} effectively, breaking down long-horizon tasks into more granular sub-tasks. We also design in-context examples with long-horizon tasks decomposed into sub-tasks. Such examples provide LLMs context on how to perform long-horizon task decomposition and generate their sub-tasks, reward functions, and their order of execution. For example: a meaningful long-horizon task in an environment with a "Mug" and "Dishwasher" is "Put the Mug in Dishwasher". The decomposition and order of this task are 1. Open the door of Dishwasher, 2. Pick Mug, 3. Put the Mug inside Dishwasher. The reward function for each would be a composition of individual terms in the above reward terms given in equation \ref{eq:reward}
% reward function: do we need to write reward function for each?

We also add language description rules to the prompt describing the available perception and control APIs from the simulator to ensure LLM doesn't produce unusable code snippets with syntax errors and unavailable API calls to mitigate the problem of hallucination in the generations. Finally, we add the query environment description to complete our prompt. The query environment description follows the same structure defined in the in-context example. 
 
 In our experiments, we find that chain-of-thought prompting is crucial for the generalization of the LLM to generate novel tasks and perform reasoning to generate meaningful reward functions. We consider both the assets we generate using the method of Section \ref{sec:assets}, as well as articulated assets from PartNet Mobility \cite{xiang2020sapien} and GAPartNet dataset \cite{gapartnet} created by human artists. We also consider the combinations of different categories of assets to perform complex long-horizon tasks. We provide a comprehensive list of our prompts on our website. We show in Section \ref{sec:experiments} that our method can generalize across assets, suggest diverse and plausible tasks, and reward functions automatically for hundreds of environments, without human involvement.
\vspace{-0.05in}

\subsection{State-based Reinforcement Learning} \label{sec:RL}
%\vspace{-0.05in}
%Following many previous works \cite{chen2022system,geng2023partmanip,pinto2017asymmetric}, 
The simulation environment provides complete state information which is highly effective in training expert policies. We train experts using reinforcement learning in our generated simulation environments using the generated reward functions to discover behaviours that solve the corresponding tasks. We use state-of-the-art Proximal Policy Optimization (PPO) \cite{schulman2017proximal}, although any RL algorithm can be used alternatively with our environments. PPO trains an actor and critic network with the objective to maximize
\begin{equation}
\mathcal{L}=\mathbb{E}\left[\frac{\pi_\theta(a \mid s)}{\pi_{\theta_{\text {old }}}(a \mid s)} \hat{A}-\epsilon K L\left[\pi_{\theta_{\text {old }}}(\cdot \mid s), \pi_\theta(\cdot \mid s)\right]\right]
\end{equation}
where $\mathbf{s}$ is the state, $\mathbf{\theta}$ is the network parameters, $\mathbf{\epsilon}$ is a hyper-parameter and $\mathbf{\hat{A}}$ is the estimated advantage. KL penalty or gradient clipping helps in stable training ensuring the new policy is close to the old one. We make use of GPU-parallel data sampling in IsaacGym\cite{issacgym} which helps in fast and stable convergence.

We use Franka Panda arm with a parallel/suction gripper as the end-effector for our tasks. The suction gripper is only used in pick-and-place tasks where grasping varied geometric objects is not possible. In all other task categories, we use parallel gripper. 

\paragraph{State / Observation Space} We model the robot state $\mathbf{S}$, the geometric details of the target part $\mathbf{b_{part}}$, and the geometric details of target asset $\mathbf{b_{asset}}$ in the environment. Robot state $\mathbf{S}$ is composed of joint angles $q p \in \mathbb{R}^{11}$, gripper position $r \in S O(3)$ and target bounding box $b_{\mathrm{part}} \in \mathbb{R}^{3 \times 8}$. 

\paragraph{Action Space}
Our action space is formulated as the gripper's target 6DoF pose at each timestep t for all tasks. We convert the end-effector pose to target joint angles by inverse kinematics IK and control the arm by position control.

%We then distill those to policies that operate directly from sensory input, so they can be deployed in the real world, following recent works \cite{chen2022system,geng2023partmanip,christen2023learning}.  
Each resulting policy that successfully learns to accomplish the task can generate trajectories that solve the task. Again, such demonstration supply is automated, without human involvement. 

% Such learned policies can be distilled into vision-language transformer policies \cite{brohan2022rt, chen2022system,geng2023partmanip,christen2023learning, jaegle2021perceiver}, so they can operate directly from visual input, without access to the object locations or poses, and we leave this to our future work.


% We specifically explore this twinsim2real pathway in our experiments. 

%Wroximal Polciy Optimization 
%[adding details of state, observation, PPO etc]
%[adding details of dagger distillation]
